Inferring Obstacles and Path Validity from Visibility-Constrained Demonstrations

Many methods in learning from demonstration assume that the demonstrator has knowledge of the full environment. However, in many scenarios, a demonstrator only sees part of the environment and they continuously replan as they gather information. To plan new paths or to reconstruct the environment, we must consider the visibility constraints and replanning process of the demonstrator, which, to our knowledge, has not been done in previous work. We consider the problem of inferring obstacle configurations in a 2D environment from demonstrated paths for a point robot that is capable of seeing in any direction but not through obstacles. Given a set of \textit{survey points}, which describe where the demonstrator obtains new information, and a candidate path, we construct a Constraint Satisfaction Problem (CSP) on a cell decomposition of the environment. We parameterize a set of obstacles corresponding to an assignment from the CSP and sample from the set to find valid environments. We show that there is a probabilistically-complete, yet not entirely tractable, algorithm that can guarantee novel paths in the space are unsafe or possibly safe. We also present an incomplete, but empirically-successful, heuristic-guided algorithm that we apply in our experiments to 1) planning novel paths and 2) recovering a probabilistic representation of the environment.

==> algo_block.tex <==
\begin{algorithm}
\SetAlgoLined
\LinesNumbered

\SetKwFunction{PolarCellDecomp}{PCD}
\SetKwFunction{ClassIdentification}{ClassID}
\SetKwFunction{IntersectDecomp}{IntersectDecomp}
\SetKwFunction{ConstructGraph}{ConstructGraph}
\SetKwFunction{CSP}{NextAssign}
\SetKwFunction{ObsParam}{ObsParam}
\SetKwFunction{CalculateGrad}{CalculateGrad}
\SetKwFunction{ConsistentConf}{ConsistentConf}

\KwIn{$\demo$\text{: the demonstration,} $\safepaths$: safe paths}
\KwOut{$O$, the environment configuration}
\BlankLine

$\spt_1, \ldots, \spt_n \leftarrow x_1, \ldots, x_n$,
$\pcds \leftarrow \{\}$, $\mathbf{\Omega} \leftarrow \{\}$

\For{$i \leftarrow 1$ \KwTo $n$}{
    $\pcd_i \leftarrow $ \PolarCellDecomp{$\demo$, $\Xi_{safe}$, $\spt_i$} \\
    %\tcp{include obs vert in class ID}
    $\Omega_i \leftarrow $ \ClassIdentification{$\pcd_i$, $x_{i+1}$} \\
    $\pcds \leftarrow \pcds \cup \pcd_i$ \\
    $\mathbf{\Omega} \leftarrow \mathbf{\Omega} \cup \Omega_i$
}
$\fullCell \leftarrow $ \IntersectDecomp{$\pcds$} \\
$G \leftarrow $ \ConstructGraph{$\fullCell$, $\spt_1, \ldots, \spt_n$} \\
\For{$i = 1$ \KwTo $\maxassign$}{
    $\assign \leftarrow $ \CSP{$G$} \\
    \For{$j=1$ \KwTo $\maxinitial$}{
        $\param \leftarrow $ \ObsParam{$\assign$} \\
        \For{$k=1$ \KwTo $\maxgrad$}{
            $\param \leftarrow \param + \grad $ \CalculateGrad{$\param$} \\
            \If{\ConsistentConf{$O(\param)$}}{
                \Return{$O(\param)$}
            }
        }
    }
}
\Return{$\emptyset$}
\caption{Find Environment Configuration}
\label{alg:find_environment_conf}
\end{algorithm}

==> notation_table.tex <==
\begin{table*}[t]
    \centering
    \rowcolors{2}{gray!25}{white}
\begin{tabular}{c|c|c}
    Notation & Note & First Location In Text \\
    \hline
    $\env$ & Environment Configuration (Obstacles) & III.A \\
    $V(t)$ & Visible area of $\X$ from the point $\xi(t)$ & III.A \\
    $R(t)$ & Known region of $\X$ up to time $t$ & III.A \\
    $F(t)$ & Known free space up to time $t$ & III.A \\
    $O(t)$ & Known obstacles up to time $t$ & III.A \\
    $U(t)$ & Unknown space up to time $t$ & III.A \\
    $\Xi$ & Set of all robot paths & III.A \\
    $\demo$ & The demonstration & III.A \\
    $\{x_1, \ldots, x_{n+2}\}$ & Vertices of the demonstration & III.A \\
    $s$ & The start in $\X$ & III.A \\
    $g$ & The goal in $\X$ & III.A \\
    $c(\cdot)$ & Cost of a robot path, always assumed to be path length & III.A \\
    $\safepaths$ & Set of safe robot paths in $\X$ & III.B \\    $\candtraj$ & A candidate robot path & III.B \\
    $\mathbb{H}^i$ & Set of all homologous classes of robot paths from vertex $x_i$ to $g$ & III.D \\
    $H^i \in \mathbb{H}^i$ & A homology class & III.D \\
    $N^i_{inf}$ & Number of paths in distinct homology classes that align with the demo & III.D \\
    $N^i_a$ & Number of alternative paths in distinct homology classes & III.D \\
    $\xi^i_{inf}$ & The inferred robot path from vertex $x_i$ & III.D \\
    $\xi^i_{a_k}$ & An alternative robot path from vertex $x_i$ & III.D \\
    $N_\spt$ & Number of survey points & III.E \\
    $\SPT$ & Set of all survey points & III.E \\
    $\spt$ & A survey point & III.E \\
    $\safeset$ & The union of the image of the safe paths and the demonstration in $\X$ & IV.A \\
    $\cell$ & A cell of $\X$ & IV.A \\
    $\class$ & A class, or a sequence of cells & IV.A \\
    $\proj\class$ & A class projection, i.e. $(\bigcup_{\cell \in \image\class}\cell) \setminus \safeset$ & IV.A \\
    $\Cell_i$ & A polar cell decomposition from survey point $\spt_i$ & IV.A \\
    $\mathbf{\Cell}$ & The collection of PCD's from each survey point & IV.A \\
    $\Class_i$ & A set of classes of the PCD $\Cell_i$ that is identified as favorable by our heuristic & IV.A \\
    $\mathbf{\Class}$ & The set of all $\Class_i$ for each PCD & IV.A \\
    $\fullCell$ & The full cell decomposition constructed by intersecting all PCD's & IV.A \\
    $G = (N,E)$ & The graph constructed on the full cell decomposition & IV.A \\
    $\assign$ & An assignment found by the CSP, i.e. $\{\graphpath_1, 
    \ldots, \graphpath_n\}$ & IV.A \\
    $q$ & Gradient step size & IV.A \\
    $\maxinitial$ & The number of initial parameterizations the algorithm will check & IV.A \\
    $\maxgrad$ & The number of gradient steps the algorithm will run & IV.A \\
    $\maxassign$ & The number of assignments of the CSP the algorithm will check & IV.A \\
    $\node$ & A node of the graph $G$ & IV.D \\
    $\nodesp\node$ & The survey point of the node & IV.D \\
    $\nodecell\node$ & The cell of the node & IV.D \\
    $\mathcal{B}$ & The boundary between two cells & IV.D \\
    $\Cell_i^{start}$ & The set of cells that contain the obstacle vertex $x_{i+1}$ & IV.D \\
    $L_{nr}$ & A function mapping a node to the nodes nearer to its survey point & IV.D \\
    $L_{fr}$ & A function mapping a node to the nodes farther from their survey point & IV.D \\
    $\nodesp{\mathcal{N}}$ & With $\mathcal{N}$ a sequence of nodes, this is a sequence of the corresponding survey points & IV.D \\
    $\nodecell{\mathcal{N}}$ & With $\mathcal{N}$ a sequence of nodes, this is a sequence of the corresponding cells & IV.D \\
    $\graphpath$ & A path on the graph $G$ & IV.D \\
    $\graphpath_{ij}$ & The longest overlap of $\graphpath_i$ and $\graphpath_j$, or $\graphpath_i$ and $\revseq{\graphpath}_j$ & IV.D \\
    $\rev$ & An indicator variable indicating if $\graphpath_j$ was reversed to obtain $\graphpath_{ij}$ & IV.D \\
    $\adj{\node_1}{\node_2}{i}$ & If $1$ then $\node_1$ and $\node_2$ are adjacent on $\graphpath_i$ & IV.D \\
    $\nu^j_i$ & A segment of $\graphpath_j$, i.e. a subsequence with the same survey point & IV.E \\
    $K^j_{seg}$ & The number of segments that comprise $\graphpath_j$ & IV.E \\
    $\zeta^j_i$ & The obstacle segment in $\X$ of the corresponding segment $\nu^j_i$ & IV.E \\
    $\beta_{l,l+1}$ & The join point of segments $\nu^j_l$ and $\nu^j_{l+1}$ & IV.E \\
    $h_{ik}$ & A family of constraint functions on the resulting obstacle & IV.E \\
    $\theta$ & The parameterization of the environment configuration & IV.E \\
    $\theta_k \in \mathbb{R}$ & a single parameter of the environment configuration & IV.E
\end{tabular}
\end{table*}
